Low dimensional interacting bosons

The theory of ultracold, dilute Bose gases is the subject of intensive studies, driven by new experimental applications, which also motivate the study of Bose-Einstein condensation (BEC) in low dimensions. From the theoretical point of view there are few, quite special, models in which we are able to prove BEC for interacting bosons. With the aim of studying the condensation problem I considered a simplified model for a three and two dimensional system of bosons interacting with a repulsive short range potential, obtained by introducing an ultraviolet momentum cutoff. I proved that the interacting theory is well defined at all orders in terms of one (in three dimensions) or two (in two dimensions) effective parameters, related to the intensity of the interaction. Moreover the correlations do not exhibit anomalous dimensions, i.e. the model is in the same universality class of the exactly soluble Bogoliubov model. The result is obtained by using Rigorous Renormalization Group techniques and implementing local Ward identities (WI), which reduce the number of independent running couplings, this fact being crucial for the control of the two dimensional theory, where the effective interactions are relevant. Since the ultraviolet momentum cutoff breaks local gauge invariance, the corrections to the formal WI have been considered.

==> flow_2d.tex <==
%\input{intro-senza-sapclass} \input{intestazione-sap} \begin{document} 


\section{The leading order beta function in $d=2$}  \label{leading_2d}

\subsection*{Role of the global WIs}

In the two dimensional case three extra global WIs are needed, in order to relate the new ``effectively marginal'' couplings $\m'_h$, $\l'_h$ and $\o_h$ to $\l_{6,h}$. These are:
\[
& \o_h = 6 \sqrt{2}\, \g^{\frac{h}{2}}\,\l_{6,h}  \\[6pt]
& 2 \sqrt{2}\, \g^{-\frac{h}{2}}\o_h -\g^{-h}\l'_h = -2\g^h \l_h  \\[6pt]
& 3\, \g^{-\frac{3}{2}h}\m'_h -2\sqrt{2} \g^{-h}\l'_h = 2 \g^{\frac{h}{2}}\m_h
\]
Assuming $\l_h$ to have a fixes point $\l_*$, in the asymptotic region \mbox{$h \arr -\io$}, since $\g^h\l_h$ and $ \g^{\frac{h}{2}}\m_h$ are going to zero,  the previous identities state that:
\[ \label{new_vertices}
& \o_h = 6 \sqrt{2}\, \g^{\frac{h}{2}}\,\l_{6,h} \non \\[6pt]
& \l'_h = 24\,\g^h \l_{6,h} \non \\[6pt]
& \m'_h = 16 \sqrt{2}\, \g^{\frac{3}{2}h} \l_{6,h}
\]
We are now ready to study the leading order flow equation for $\l_h$ and $\l_{6,h}$. 
%and prove the assumption on their behavior. 
Under the previous assumption on $\l_h$ the order in the small parameters $\l$ and $\e=\l \r_0 R_0^2$ in the asymptotic region is given by:
\[ \label{asym_2d}
\tl{C}_{2d}(P_v; \l, \e)  =   \r_0 R_0^{-2} &\, \l^{1-\frac{1}{2}(n_l^\txe+n_t^\txe)}\,\e^{-2 +\frac{3}{2}n_l^\txe+ \frac{1}{2}n_t^\txe + \frac{1}{2}n_\dpr^\txe} 
\non \\[6pt]
&  \, (\l \l_*)^{m_{4}+\frac{1}{2}m_{3}}\,(\e \n_*)^{m_{2}}\,  (\l \e^{-1} \,\l \l_{6})^{m_6}\non \\[6pt]
& \lft(\l \e^{-1} \,\frac{\l_{6}}{\l_*}\rgt)^{m'_4}\,\lft( \l \e^{-2} \, \frac{\l^2_{6}}{\l_*^3}\rgt)^{\frac{1}{2}m'_3} \,\lft( \e \, \frac{\l^2_{6}}{\l_*}\rgt)^{\frac{1}{2}m'_5}
\non \\[6pt]
& \lft(\e^{-1}\g^h \l_* \rgt)^{\frac{1}{2}(m_3 + m_5 + 2m'_4 +3m'_3)- n_{ll}}
\]
The leading order diagrams are the one loop diagram (remind that the loop number is equal to $L=m_4 + m'_4 + (m_3+m'_3)/2 +3m_5/2 +2m_6 -n^\txe/2 +1$) where all the internal dashed legs are contracted among them, in order to minimize the exponent of $\g^h$, on the last line of \eqref{asym_2d}. 



\feyn{
\begin{fmffile}{feyn-TESI/zeta2d}
 \unitlength = 0.8cm
\def\myl#1{2.5cm}
\begin{align*}
\parbox{\myl}{\centering{
		\begin{fmfgraph*}(2,1.1)
			\fmfleft{i1}
			\fmfright{o1}
			\fmf{dashes}{i1,v1,o1}
			\fmfv{label={$Z_{h-1}/2$},label.angle=90,label.dist=-0.4w}{v1} 
                   \bBall{v1}
		\end{fmfgraph*}
		}}
		& =
		\parbox{\myl}{\centering{
		\begin{fmfgraph*}(2,1)
			\fmfleft{i1}
			\fmfright{o1}
			\fmf{dashes}{i1,v1,o1}
			\fmfv{label={$Z_h/2$},label.angle=-90}{v1} 
                   \Ball{v1}
		\end{fmfgraph*}
	}}			-\;
\parbox{\myl}{\centering{
		\begin{fmfgraph*}(2.2,1.5) \fmfkeep{z1}
			\fmfleft{i1}
			\fmfright{o1}
			\fmf{dashes}{i1,v1,o1}
                    \fmf{plain}{v1,v1}
                    \Ball{v1}
		\end{fmfgraph*}
	}}			+\;
	\parbox{\myl}{\centering{
			\begin{fmfgraph*}(2.5,1.4)  \fmfkeep{z2}
			\fmfleft{i1}
			\fmfright{o1}
			\fmf{dashes, tension=1.5}{i1,v1}
			\fmf{plain,left=0.7, tension=0.4}{v1,v2}
			\fmf{plain,right=0.7, tension=0.4}{v1,v2}
			\fmf{dashes}{o1,v2}
			\Ball{v1,v2}
			\end{fmfgraph*}  
			}}   
	+\;
	\parbox{\myl}{\centering{
			\begin{fmfgraph*}(2.5,1.4) \fmfkeep{z3}
			\fmfleft{i1}
			\fmfright{o1}
			\fmf{dashes, tension=1.5}{i1,v1}
			\fmf{dashes,left=0.7, tension=0.4}{v1,v2}
			\fmf{dashes,right=0.7, tension=0.4}{v1,v2}
			\fmf{dashes}{o1,v2}
			\Ball{v1,v2}
			\end{fmfgraph*}  
			}}  
\end{align*}
\end{fmffile}	
}{{\bf Beta function for $Z_h$, d=2.} }{zeta2d}

\subsection{Beta function for $\l_h$ }

In spite of studying directly the leading order beta function $\b_h^\l$ for $\l_h$ it results more convenient to look at the beta function $\b_h^Z$ of $Z_h$, which a smaller number of diagram  contribute to, and then use the global WI
\[
Z_h = 16 \g^h \l_h
\]
to obtain the flow equation for $\l_h$: 
\[
\g^{h-1}\l_h-1 = \g^h\l_h + \g^h\b_h^\l
\]
with $\g^h\b^\l_h=\b^Z_h/16$. The leading order diagrams contributing to the flow of $Z_h$ according to \eqref{asym_2d} are showed in fig. \ref{zeta2d}. In the following we will denote as:
\[ \label{beta_def}
&\b^{2d}_0 = \frac{1}{(2\pi)^3}\int dk_0 d^2\kk \,f_0(k_0^2 +\kk^2)  
= \frac{1}{2\pi^2}\,\sqrt{\tfrac{2}{\g^2+1}} \,\tfrac{2(\g^3-\g^{-3})}{3(\g^2+1)}
\non \\[6pt]
%
& \b^{2d}_1 = \frac{1}{(2\pi)^3}\int dk_0 d^2\kk \,\frac{f_0(k_0^2 +\kk^2)}{k_0^2 +\kk^2}  = \frac{1}{2\pi^2}\,\sqrt{\tfrac{2}{\g^2+1}} \,\g^{-1}(\g^2-1)
\non \\[6pt]
%
&\b^{2d}_2 = \frac{1}{(2\pi)^3}\int dk_0 d^2\kk \,\frac{f_0(k_0^2 +\kk^2)}{(k_0^2 +\kk^2)^2}  = \frac{1}{2\pi^2}\,\sqrt{\tfrac{2}{\g^2+1}} \,\tfrac{\g^{2}+1}{2}(\g-\g^{-1})
\non \\
\]  \nota{spostare calcoli a dopo, scrivendo che ho usato un gradino per fare i conti}
with $f_0(k)$ a $C^\io$ regularization of the characteristic function of the set $$\lft[\sqrt{\tfrac{2}{1+\g^2}}\,\g^{-1}, \sqrt{\tfrac{2}{1+\g^2}}\,\g \rgt]$$
The behavior of the asymptotic propagator is
\[
g^{(h)}_{\a \a'}(x) & = (\r_0 R_0^2)^{-1} \frac{1}{(2\pi)^3}\int dk_0 d^2\kk\, f_h(k_0^2 +\e\kk^2)\, g^{(h)}_{\a \a'}(k) \non \\[6pt]
g^{(h)}_{\a \a'}(k) & = 
\left(\begin{array}{cc}
Z_h   & - \frac{k_{0}}{k_0^2 +\e\kk^2}\\
\frac{k_{0}}{k_0^2 +\e\kk^2} & \quad \frac{\e}{k_0^2 +\e\kk^2}
\end{array}\right)
\]
where the first line and row correspond to $a=l$ and the second line and row correspond to $\a'=t$. The values of the diagrams of picture \ref{zeta2d} are calculated below. The combinatorial factors take into account: 
\begin{enumerate}[a.]
\item the coefficient of the truncated expectations, which is $(-1)^{n+1}/n!$ if we are contracting $n$ vertices;
\item the different possibilities of choosing different vertices between those present in the expectations, giving rise to the same graph;
\item for each vertex, the different possibilities of choosing the external lines;
\item the different possibility of contracting the internal lines.
\end{enumerate}
\feynH{
 \unitlength = 0.8cm
\def\myl#1{2.5cm}
\begin{align*}
\parbox{\myl}{\centering{\fmfreuse{z1}}}
 & = \; \l \e^{-1}\,\b^{2d}_1\,\l'_h = \; 24\, \l \e^{-1}\,\b_1^{2d}\g^h\,\l_{6,h}   \non \\[6pt]
\parbox{\myl}{\centering{\fmfreuse{z2}}} &= \; -\frac{1}{2!}\,2\,\l\,\b^{2d}_2\, \m_h^2 = \; -32\,\l\,\b^{2d}_2 \g^h\,\l_h^2  \non \\[6pt]
 \parbox{\myl}{\centering{\fmfreuse{z3}}} &=\; -\frac{1}{2!}\,2\cdot 3^2\,\l\e^{-2}\,\b^{2d}_0\, \lft(\frac{\m'_h}{Z_h}\rgt)^2 =\; -18\,\l\e^{-2}\,\b^{2d}_0\,\g^h\,\lft(\frac{\l_{6,h}}{\l_h}\rgt)^2
\end{align*}
}
Then, 
\[ \label{lambda_1}
\g^{-1}\l_{h-1} - \l_h= - \l \,(1-\g^{-1})\,\lft( 4\,\tl{\b}^{2d}_2\,\l_h^2 \;-\; 3\,\tl{\b}_1^{2d}\,\e^{-1}\l_{6,h} \;+\; \frac{9}{4}\,\tl{\b}^{2d}_0 \lft(\frac{\l_{6,h}}{\e \l_h}\rgt)^2 \rgt)
\]
with $(1-\g^{-1}) \tl{\b}^{2d}=\b^{2d}$. Assuming $\l_{6,h}$ to reach a fixed point 
\[
\l_6 = c_6\,\e\l_*^2
\]
 with $c_6$ a positive constant the \eqref{lambda_1} becomes
\[
\l_* = \frac{\l^{-1}}{4\,\tl{\b}^{2d}_2-\; 3\,c_6\,\tl{\b}_1^{2d} + \frac{9}{4}\,c^2_6\,\tl{\b}^{2d}_0 }
%\lft(4\,\tl{\b}^{2d}_2 +\; 3\,c_6\,\tl{\b}_1^{2d} + \frac{9}{4}\,c^2_6\,\tl{\b}^{2d}_0  \rgt)^{-1} \l^{-1}
\]

\feyn{
\begin{fmffile}{feyn-TESI/muprimo2d}
 \unitlength = 0.8cm
\def\myl#1{2.3cm}
\begin{align*}
\parbox{\myl}{\centering{
		\begin{fmfgraph*}(2,1.5)
			\fmfleft{i1}
			\fmfright{o1,o2}
			\fmf{dashes, tension=1.5}{i1,v1}
                    \fmf{dashes}{o1,v1,o2}
			\fmfv{label={$\m'_{h-1}$},label.angle=90,label.dist=-0.4w}{v1} 
                   \bBall{v1}
		\end{fmfgraph*}
		}}
		& =
		\parbox{\myl}{\centering{
		\begin{fmfgraph*}(2,1.5)
                   \fmfleft{i1}
			\fmfright{o1,o2}
			\fmf{dashes, tension=1.5}{i1,v1}
                   \fmf{dashes}{o1,v1,o2}
			\fmfv{label={$\m'_h$},label.angle=-90}{v1} 
                   \Ball{v1}
		\end{fmfgraph*}
	}}			-\;
\parbox{\myl}{\centering{
		\begin{fmfgraph*}(2.2,1.5) \fmfkeep{m1}
			\fmfleft{i1}
			\fmfright{o1,o2}
			\fmf{dashes, tension=1.5}{i1,v1}
                   \fmf{dashes}{o1,v2}
                   \fmf{dashes}{o2,v3}
			\fmf{plain, right=0.4, tension=0.6}{v1,v2}
                    \fmf{plain, left=0.4, tension=0.6}{v1,v3}
                   \fmf{plain, right=0.4, tension=0.2}{v2,v3}
                    \Ball{v1,v2,v3}
		\end{fmfgraph*}
	}}			+\;
	\parbox{\myl}{\centering{
		\begin{fmfgraph*}(2.2,1.5) \fmfkeep{m2}
			\fmfleft{i1}
			\fmfright{o1,o2}
			\fmf{dashes, tension=1.5}{i1,v1}
                   \fmf{dashes}{o1,v2}
                   \fmf{dashes}{o2,v3}
			\fmf{dashes, right=0.4, tension=0.6}{v1,v2}
                    \fmf{dashes, left=0.4, tension=0.6}{v1,v3}
                   \fmf{dashes, right=0.4, tension=0.2}{v2,v3}
                    \Ball{v1,v2,v3}
		\end{fmfgraph*}
	}}			+\;
	\parbox{\myl}{\centering{
			\begin{fmfgraph*}(2.2,1.5) \fmfkeep{m3}
			\fmfleft{i1}
			\fmfright{o1,o2}
			\fmf{dashes, tension=1.5}{i1,v1}
			\fmf{plain,left=0.7, tension=0.4}{v1,v2}
			\fmf{plain,right=0.7, tension=0.4}{v1,v2}
			\fmf{dashes}{o1,v2,o2}
			\Ball{v1,v2}
			\end{fmfgraph*}  
			}}  
\end{align*}
\end{fmffile}	
}{{\bf Beta function for $\m'_h$, d=2.} }{muprimo2d}


\subsection{Beta function for $\l_{6,h}$}

Similarly at what happens for $\l_h$, the beta function for $\l_{6,h}$ may be rewritten in term of the beta function of $\m'_h$, using the last of \eqref{new_vertices}: 
\[
\l_{6,h-1} = \l_{6,h} +\b_h^{\l_6}
\]
with $\b^{\l_6}_h=\g^{-\frac{3}{2}h} \b^{\m'}_h/(16 \sqrt{2})$. The leading order diagrams contributing to the flow of $\m'_h$ are showed in fig. \ref{muprimo2d}. Let's calculate them:
\feynH{
 \unitlength = 0.8cm
\def\myl#1{2.5cm}
\begin{align*}
\parbox{\myl}{\centering{\fmfreuse{m1}}}
 & = \; +\frac{1}{3!}\cdot 6  \, \l \e \,\b^{2d}_3\,\m^3_h =   
 2^7\sqrt{2}\, \g^{\frac{3}{2}h}\,\b^{2d}_3\,\l \e\,\l^3_h 
\non \\[6pt]
%
\parbox{\myl}{\centering{\fmfreuse{m2}}} &= \; +\frac{1}{3!}\,3^3\cdot 6\,\l \e^{-2}\,\b^{2d}_0\, \lft(\frac{\m'_h}{Z_h}\rgt)^3 
= \; 3^3 \cdot 2\sqrt{2} \,\g^{\frac{3}{2}h}\,\b^{2d}_0\,\l \e\, \lft(\frac{\l_{6,h}}{\e \l_h}\rgt)^3 
 \non \\[6pt]
% 
\parbox{\myl}{\centering{\fmfreuse{m3}}} &=\; -\frac{1}{2!}\cdot 2 \cdot 2 \, \l \,\b^{2d}_2\,\l'_h\,\m_h =   
-3\cdot 2^6\sqrt{2}\, \g^{\frac{3}{2}h}\,\b^{2d}_2\,\l\,\l_h\,\l_{6,h} 
\end{align*}
}
where
\[
&\b^{2d}_3 = \frac{1}{(2\pi)^3}\int dk_0 d^2\kk \,\frac{f_0(k_0^2 +\kk^2)}{(k_0^2 +\kk^2)^3}  = \frac{1}{2\pi^2}\,\sqrt{\tfrac{2}{\g^2+1}} \,\tfrac{(\g^{2}+1)^2}{12}(\g^3-\g^{-3})
\]
Then, 
\[ \label{l6_1}
\l_{6,h-1} - \l_{6,h} &=  8\,\b^{2d}_3 \l \e\,\l^3_h -  12\,\b^{2d}_2\,\l \l_h\,\l_{6,h} 
+\frac{27}{8}\,\b^{2d}_0\,\l \e\, \lft(\frac{\l_{6,h}}{\e \l_h}\rgt)^3  \non \\[6pt]
& = \l \l_h \biggl[ \, 8\b^{2d}_3\,\e \l_h^2 - \l_{6,h} \lft(12\,\b^{2d}_2 - \frac{27}{8}\,\b^{2d}_0\, \Bigl(\frac{\l_{6,h}}{\e \l^2_h}\Bigr)^2 \rgt) \biggr] 
\]

%With the assumption $ \l_6 = c_6\,\e\l_*^2$ the fixed point equation is satisfied for
\vskip 2cm

\[
\l_{h-1} - \g\l_h &= - \l \,(\g-1)\,\l_h^2\,\lft( 4\,\tl{\b}^{2d}_2\;-\; 3\,\tl{\b}_1^{2d}\,\lft(\frac{\l_{6,h}}{\e \l_h^2}\rgt) \;+\; \frac{9}{4}\,\tl{\b}^{2d}_0 \lft(\frac{\l_{6,h}}{\e \l^2_h}\rgt)^2 \rgt)  \non \\[12pt]
\l_{6,h-1} - \l_{6,h} &=  (1-\g^{-1})\,\e\l  \l_h^3\, \lft[ \, 8\tl{\b}^{2d}_3 -12\,\tl{\b}^{2d}_2 \lft(\frac{\l_{6,h}}{\e \l^2_h}\rgt)  + \frac{27}{8}\,\tl{\b}^{2d}_0\, \lft(\frac{\l_{6,h}}{\e \l^2_h}\rgt)^3 \rgt]  \non
\]

%\section{Global WIs in the asymptotic region}

\feyn{
\begin{fmffile}{feyn-TESI/GWI_2d}
 \unitlength = 0.8cm
\def\myl#1{2.3cm}
\begin{align*}
\parbox{\myl}{\centering{ \vskip 0.8cm
			\begin{fmfgraph*}(2.2,1.3) 
			\fmfleft{i1}
			\fmfright{o1}
			\fmf{dashes, tension=1.2}{i1,v1}
			\fmf{plain,left=0.7, tension=0.4}{v1,v2}
			\fmf{plain,right=0.7, tension=0.4}{v1,v2}
			\fmf{dashes, tension=1.2}{o1,v2}
			\Ball{v1,v2}
			\end{fmfgraph*}    \\[3pt]
                   $ -\frac{1}{2!} \cdot 2 $
			}} 
& = \quad 8 \parbox{\myl}{\centering{ \vskip 0.8cm
			\begin{fmfgraph*}(2.2,1.3)
			\fmfleft{i1,i2}
			\fmfright{o1,o2}
			\fmf{plain, tension=1.2}{i1,v1,i2}
			\fmf{plain,left=0.7, tension=0.4}{v1,v2}
			\fmf{plain,right=0.7, tension=0.4}{v1,v2}
			\fmf{plain, tension=1.2}{o1,v2,o2}
			\Ball{v1,v2}
			\end{fmfgraph*}  
 			  \\[3pt]    $ -\frac{1}{2!}\,\binom{4}{2}^2 \, 2 $
			}} +\; 8
 \parbox{\myl}{\centering{ \vskip 0.8cm
		\begin{fmfgraph*}(2.2,1.3) 
			\fmfleft{i1,i2}
			\fmfright{o1,o2}
			\fmf{plain, tension=1.5}{i1,v1,i2}
                   \fmf{plain}{o1,v2}
                   \fmf{plain}{o2,v3}
			\fmf{plain, right=0.4, tension=0.6}{v1,v2}
                    \fmf{plain, left=0.4, tension=0.6}{v1,v3}
                   \fmf{dashes, right=0.4, tension=0.2}{v2,v3}
                    \Ball{v1,v2,v3}
		\end{fmfgraph*}
            \\[3pt] $ \frac{1}{3!}\,3\,\binom{4}{2}\,\binom{2}{1}^2\,2 $
	}} +\; 8
\parbox{\myl}{\centering{  \vskip 0.8cm
			\begin{fmfgraph*}(2.2,1.3) 
			\fmfleft{i1,i2}
			\fmfright{o1,o2}
			\fmf{plain, tension=1.8}{i1,v1}
                    \fmf{plain, tension=1.8}{i2,v2}
                    \fmf{plain}{v1,v2}
                    \fmf{dashes}{v2,v4}
                    \fmf{dashes}{v1,v3}
                    \fmf{plain}{v4,v3}
			%\fmf{dashes,left=0.7, tension=0.4}{v1,v2}
			%\fmf{dashes,right=0.7, tension=0.4}{v1,v2}
			\fmf{plain, tension=1.8}{o1,v3}
	             \fmf{plain, tension=1.8}{v4,o2}
			\Ball{v1,v2,v3,v4}
			\end{fmfgraph*}  
                    \\[3pt] $ -\frac{1}{4!}\,\binom{4}{2}\,2 $
			}} \\[12pt]
%------------------------------------------------------------------------
\parbox{\myl}{\centering{ \vskip 0.4cm
		\begin{fmfgraph*}(2,2)
			\fmfleft{i1}
			\fmfright{o1}
			\fmf{plain}{v1,v1}
                    \fmf{dashes}{i1,v1,o1}
                   \Ball{v1}
		\end{fmfgraph*}
             \\[-3pt] $1$
		}}
		& = \quad 8
		\parbox{\myl}{\centering{  \vskip 0.8cm
             \vskip -0.5cm
		\begin{fmfgraph*}(2,2)
                   \fmfright{i1}
                   \fmfleft{i2}
			\fmfbottom{o1,o2}
			\fmf{plain, tension=1.5}{i1,v1,i2}
                   \fmf{plain}{o1,v1,o2}
			\fmf{plain}{v1,v1}
                   \Ball{v1}
		\end{fmfgraph*}
 		\\[3pt] $  \binom{6}{2}$
	}}		
		+\; 8
	\parbox{\myl}{\centering{ \vskip 0.8cm
		\begin{fmfgraph*}(2.2,1.3) 
			\fmfleft{i1,i2,i3}
			\fmfright{o1}
			\fmf{plain, tension=1.2}{i1,v1,i2}
                   \fmf{plain, tension=1.2}{i3,v1}
                   \fmf{plain, tension=1.8}{v2,o1}
			\fmf{dashes, right=0.7, tension=0.6}{v1,v2}
                    \fmf{plain, left=0.7, tension=0.6}{v1,v2}
                    \Ball{v1,v2}
		\end{fmfgraph*}
             \\[3pt] $  -\frac{1}{2!}\,2\,\binom{5}{1}\,\binom{2}{1}\,2$
	}}		+\; 8\;\parbox{\myl}{\centering{ \vskip 0.8cm
		\begin{fmfgraph*}(2.2,1.3) 
			\fmfleft{i1,i2}
			\fmfright{o1,o2}
			\fmf{plain, tension=1.5}{i1,v1,i2}
                   \fmf{plain}{o1,v2}
                   \fmf{plain}{o2,v3}
			\fmf{dashes, right=0.4, tension=0.6}{v1,v2}
                    \fmf{dashes, left=0.4, tension=0.6}{v1,v3}
                   \fmf{plain, right=0.4, tension=0.2}{v2,v3}
                    \Ball{v1,v2,v3}
		\end{fmfgraph*}
                \\[3pt] $  \frac{1}{3!}\,3\,\binom{2}{1}^2\,2$
	}}
	  \\[12pt]
%---------------------------------------------------------------------------
\parbox{\myl}{\centering{ \vskip 0.8cm
			\begin{fmfgraph*}(2.2,1.3) 
			\fmfleft{i1}
			\fmfright{o1}
			\fmf{dashes, tension=1.2}{i1,v1}
			\fmf{dashes,left=0.7, tension=0.4}{v1,v2}
			\fmf{dashes,right=0.7, tension=0.4}{v1,v2}
			\fmf{dashes, tension=1.2}{o1,v2}
			\Ball{v1,v2}
			\end{fmfgraph*}  
  			\\[3pt] $  -\frac{1}{2!}\,\binom{3}{2}^2\,2$
			}}  & = \quad 8
	\parbox{\myl}{\centering{  \vskip 0.8cm
			\begin{fmfgraph*}(2.2,1.3) 
			\fmfleft{i1,i2}
			\fmfright{o1,o2}
			\fmf{plain, tension=1.5}{i1,v1,i2}
			\fmf{dashes,left=0.7, tension=0.4}{v1,v2}
			\fmf{dashes,right=0.7, tension=0.4}{v1,v2}
			\fmf{plain}{o1,v2,o2}
			\Ball{v1,v2}
			\end{fmfgraph*}  
			\\[3pt] $  -\frac{1}{2!}\,2$
			}} 
%------------------------------------------------------------------------
\end{align*}
\end{fmffile}	
}{{\bf Asymptotic global WI $Z_h=16\l_h$, d=2.} The sum of the diagrams on the l.h.s. represent the leading order beta function of $Z_h/2$ in the asymptotic region $h \arr \io$; the sum of the diagrams on the r.h.s. side is the leading order beta function of $\l_h$. Using \blue{vecchie WI} and \eqref{new_vertices} one can check that the global WI is satisfied among diagrams with the same number of plain (\ie transverse) propagators. }{GWI_2d}

\[ 
&\tl{\b}^{2d}_0 = \frac{1}{2\pi^2}\,\sqrt{\tfrac{2}{\g^2+1}} \,\tfrac{2}{3} \tfrac{(\g^2+\g+1)(\g^3+1)}{\g^2(\g^2+1)}
&
%
& \tl{\b}^{2d}_1 =  \frac{1}{2\pi^2}\,\sqrt{\tfrac{2}{\g^2+1}} \,(\g+1)
\non \\[6pt]
%
&\tl{\b}^{2d}_2  = \frac{1}{2\pi^2}\,\sqrt{\tfrac{2}{\g^2+1}} \,\tfrac{\g^{2}+1}{2}\,(\g+1)
&
& \tl{\b}^{2d}_3 = \frac{1}{2\pi^2}\,\sqrt{\tfrac{2}{\g^2+1}} \,\tfrac{(\g^{2}+1)^2}{12}\tfrac{(\g^2+\g+1)(\g^3+1)}{\g^2}
\] 

\subsection*{Appendice A}

The bound for a generic diagram $\G$ where all the vertices are at scale $h_* \ll \bh$ turns out to be
\[  \label{2d_hstar}
\tl{C}^{(h_*)}_{2d}(P_v;\e, \r_0, R_0)  \leq &\; \cst \,\r_0 R_0^{-2}  \l^{1-\frac{1}{2}(n_l^\txe+n_t^\txe)}\,\e^{-2 +\frac{3}{2}n_l^\txe+ \frac{1}{2}n_t^\txe + \frac{1}{2}n_\dpr^\txe} 
\non \\[6pt]
&  \, \lft[\l \l_{h_*} \rgt]^{m_{4}+\frac{1}{2}m_{3}}\,(\e \n_h)^{m_{2}}\,  \lft[(\l \l_h)^2 \,\frac{\l_{6,h_*}}{\e \l^2_h}\rgt]^{m_6}\non \\[6pt]
%
&\,\lft[\, \l \l_{h_*} \,\frac{\l_{6,h_*}}{\e \l_h^2} \,\rgt]^{m'_4} 
\,\lft[\, (\l \l_{h_*})^{\frac{1}{2}} \,\frac{\l_{6,h_*}}{\e \l_h^2} \,\rgt]^{m'_3}
\,\lft[\, (\l \l_{h_*})^\frac{3}{2} \,\frac{\l_{6,h_*}}{\e \l_h^2} \,\rgt]^{m'_5}
\non \\[6pt]
%
& \lft(\e^{-1}\g^h \l_* \rgt)^{\frac{1}{2}(m_3 + m_5 + 2m'_4 +3m'_3)- n_{ll}} \non \\
\]

%\end{document}
